G3Ego: Gaze-Guided Graphs for Egocentric Action Understanding

Egocentric action understanding is often addressed using large video models pretrained on extensive exocentric datasets. However, many first-person actions depend on a small number of hand-object interactions involving only a few relevant entities. We propose G3Ego, a graph-based framework for egocentric action understanding that uses gaze as a structural cue to identify action-relevant entities in the scene. From sparsely sampled frames, G3Ego constructs action scene graphs from vision-language descriptions, grounded objects, and hand cues, and then prunes irrelevant entities using the camera wearer's gaze. The resulting graph embeddings are temporally aggregated for action recognition and anticipation. Unlike prior work that uses gaze primarily as an auxiliary modality or attention signal, G3Ego incorporates gaze directly into graph construction, producing efficient and interpretable representations focused on action-relevant interactions. Experiments on EGTEA Gaze+ and MECCANO show that G3Ego achieves competitive performance compared with video-based approaches and consistently improves Macro-F1 under class-imbalanced evaluation, while avoiding reliance on computationally expensive video pretraining. These results demonstrate the effectiveness of gaze-guided graph representations for egocentric action understanding.

==> sections/extra/4_methodology_old.tex <==
\section{GPASG method}
Given a sample video, N frames representing a video, we first represent frame, build a graph, prune it base don a gze, and then we aggregate the representation for the set of frames. 

1. Frame representation
Global descriptors in the form of global embeddings and caption and local descriptors objects and hands.

2. Graph construction (full graph) 

3. Gaze guided pruning 

4. Temporal graph modelling 
Graph embedder and Temporal Aggregation 




\begin{figure}[!t]
    \centering
    \fbox{
        \begin{minipage}[c][0.25\textheight][c]{0.95\columnwidth}
            \centering
            \vspace{1em}
            \textbf{Framework figure}
            \vspace{1em}
        \end{minipage}
    }
    \caption{\textbf{Framework figure}}
    \label{fig:motivation_framework}
\end{figure}


We propose \emph{Full Action Scene Graphs} (FASG), visualized inFig.~\ref{fig:fasg}, and \emph{Gaze-Pruned Action Scene Graphs} (GPASG), visualized in Fig.~\ref{fig:gpasg}, for temporal understanding of activities in egocentric videos. Section~\ref{sec:asg} introduces the ASG formulation and the overall pipeline.  Section~\ref{par:graph_variants} describes the two graph variants, FASG and GPASG. Section~\ref{sec:graph_construction} details our graph construction procedure.  Section~\ref{sec:graph_representations} explains how graphs are encoded into fixed-size embeddings. Finally, Section~\ref{sec:graph_model} presents our attention-based graph model for activity recognition.


\subsection{Action Scene Graph Definition}
\label{sec:asg}

\paragraph{Action Scene Graph}
\label{par:action_scene_graphs}
Action scene graphs (ASGs) are structural representations of actions, defined by action verb(s), interacting objects with corresponding attributes, and semantic relations between each.
Formally, for each action clip we construct an ASG $\mathcal{G}_t = (\mathcal{V}_t, \mathcal{E}_t)$,
where $\mathcal{V}_t$ contains a main action verb node $v_t$, optional auxiliary verb nodes $\tilde{v}_t$, and a set of object nodes $\mathcal{O}_t$ (direct and auxiliary objects).
Each object node $o \in \mathcal{O}_t$ is associated with a set of attributes $\mathcal{A}(o)$ and a corresponding bounding-box feature vector $\mathbf{f}(o)$.
Additionally, each clip is represented by a frame-level visual feature $\mathbf{x}_t$ extracted by a frozen vision encoder.
Edges $\mathcal{E}_t$ encode semantic relations, including verb - object interactions (e.g., direct object and gazed at object), auxiliary verb - main verb dependencies, and prepositional relations. Following previous work~\cite{easg2024}, we define each ASG as the triplet
$\mathcal{G}_t = (\mathcal{V}_t, \mathcal{E}_t, \mathbf{X}_t)$, set of which serves as a concise graph summary of the action clip.

\paragraph{Graph variants}
\label{par:graph_variants}
We differentiate two graph variants. A \emph{full ASG (FASG)} contains all detected objects within the scene, whereas a \emph{gaze pruned action scene graph (GPASG)}, further defined in \ref{par:graph_pruning}, retains only those objects that are located within the wearer’s gaze region or are action critical (direct object), where the latter is determined from the VLM annotation, where the gazed-at object is determined by absolute Euclidean distance between ground truth gaze coordinates mapped to closest bounding box coordinates obtained from the object detector. The purpose of pruning is to avoid background clutter and obtain a compact scene representation. Examples of a FASG  and GPASG are shown in Fig.~\ref{}. Following common nomenclature, such graphs are with no constraint, meaning they are not limited to single verb - object relationship.

\paragraph{Graph pruning}
\label{par:graph_pruning}
Global efficiency is measured across the graph, whereas local efficiency is measured per node. Our pruning algorithms can be viewed as improving global communication by shortening the longest path in the graph. Local efficiency is not meaningful for our star-shaped graphs due to their limited connectivity between nodes and the absence of triangles.

Since the ARIA Everyday Activities dataset~\cite{lv2024aria} provides gaze annotations for each frame in the form of $(x,y)$ coordinates, we directly incorporate gaze information into our pipeline to prune action scene graphs. Motivated by prior work on gaze-guided activity recognition, we use gaze to retain objects within the camera wearer’s gaze region while removing background and less relevant objects.

Gaze based pruning offers several advantages:
(a) explicit encoding of gaze, providing the model with information about what the person is looking at;
(b) shortening the longest path across the graph; and
(c) requiring fewer parameters and fewer (often scarce) per-frame labels during training.

We support this claim by measuring the maximum shortest path distance between the camera wearer node and the furthest node in the graph, as well as global efficiency. 

Global efficiency is measured by the following formula 
\[
E_{\mathrm{glob}}(G) = \frac{1}{n(n-1)} \sum_{i \neq j} \frac{1}{d_{ij}}
\] where $n$ is the number of nodes and $d_{ij}$ is the shortest path distance between nodes $i$ and $j$. 

Maximum shortest path from the camera wearer node is defined as 
\[
D_{\max} = \max_{v \in \mathcal{V},\, v \neq v_{cw}} d(v_{cw}, v)
\]
where $v_{cw}$ denotes the camera wearer node and $d(\cdot,\cdot)$ denotes the shortest path distance.


The average maximum shortest-path length in FASG is 2.06, with an average global efficiency of 0.59, compared to 2.0 and 0.78 for GPASG. This is expected due to our star shaped graphs; gaze pruning removes auxiliary verbs and any further objects (nodes) and relations (edges) other than the camera wearer, main verb and up to two objects. Therefore, the maximum path in such a graph is 2, if both direct and gazed-at object are added. As for global efficiency, given distance between any two nodes is larger in FASG with addition of other relations and objects, it is expected that efficiency is higher due to shorter paths for the information to flow between any two nodes in the graph. For further visualization, we include action annotation, FASG and GPASG annotations and respective measures to better present the intuition behind these metrics.

\subsection{Action Scene Graph Construction}
\label{sec:graph_construction}
This subsection describes how the components introduced in Section~\ref{sec:asg} are used to construct ASGs from raw egocentric video. A visualization of our workflow is shown in Figure~\ref{}. 

\textbf{Frame level feature extraction}
\label{par:feature_extraction}
We obtain frame-level features (clip features) using DINOv3-huge/16+~\cite{dinov3_2023} to compute per-frame feature representations that are used as the main feature in action scene graphs.

\paragraph{Action and activity annotation pipeline}
\label{par:action_act_annotation}
To avoid dense frame processing, we employ uniform sampling at the 3 second clip level to produce a set of key frames. The key frames are grouped over a temporal window of 30 seconds into 10 frames for activity recognition, with no overlap between windows. We argue that each key frame represents a meaningful standalone action and is action annotated using VLM, while each set of 10 consecutive frames is activity annotated using the same VLM. Therefore, we assume one action is being performed and annotated across 30 seconds. We use the LLaVA-34B vision language model~\cite{llava2023} to generate action descriptions for each clip and activity annotations for a set of 10 consecutive frames. The resulting captions are parsed using spaCy~\cite{honnibal2020spacy} to extract grammatical structure (e.g. verbs, auxiliary verbs, direct objects, prepositional relations), which is used for subsequent graph construction.

\paragraph{VLM annotation parsing}
\label{par:vlm_ann_parse}
To represent each clip semantically, we construct action scene graphs (ASGs) following the design of~\cite{easg2024,easgbench2025}. We first parse VLM annotations to obtain the following categories: direct object, auxiliary object, object attributes, auxiliary verbs, and object - verb relations (for both the main verb and the auxiliary verb). We remove the need to have three frames (before, during, and after the action) as in~\cite{easg2024,easgbench2025}, and we remove hand nodes. Each graph contains a \emph{wearer node}, a \emph{verb/action node}, an \emph{auxiliary verb/action node} if present, and a set of \emph{object nodes}. Edges encode semantic relations such as direct-object dependency, main action verb to auxiliary verb dependency, prepositional modifiers, and verb - object interactions. Verb - object interactions are further dissected into objects that the main verb interacts with, and objects that the auxiliary verb interacts with.

\paragraph{VLM annotation post-processing}
\label{par:vlm_ann_postprocess}
We collect all relations, attributes, objects, and verbs present in our annotations. We further ensure that compound nouns are treated as a separate class, while descriptive compounds consisting of an adjective and a noun are dissected into a base object and attribute pairs. For instance, \emph{board game} is kept as is, with the base object being \emph{board game} and no attributes, while \emph{white doors} is split into \emph{door} as the base object and \emph{white} as an attribute. This is done in the VLM annotation parsing pipeline, as part of annotation refinement, using dependency parses obtained with spaCy. By examining word dependencies, it is possible to determine, with reasonable confidence, whether a phrase forms a compound noun.

Following these annotations, each graph encodes prepositional relations as edges, as well as object attributes. The result is a multi-hot representation. We encode object attributes and relations as multi-hot matrices of size $|\mathcal{O}|\times|\mathcal{A}|$ and $|\mathcal{O}|\times|\mathcal{R}|$, respectively.

\paragraph{Parsed object visual grounding}
\label{par:visual_grounding}
 We construct a descriptive list of objects per frame (base object + attributes), and use GroundingDINO-T~\cite{groundingdino2023} for visual grounding and as bounding box feature extractor. We choose it as it is an open-vocabulary model, enabling semantic differentiation of objects using our object attributes.  Each object receives one bounding box feature; if multiple instances are detected, mean pooling is performed within the frame (not across frames). To maintain an efficient pipeline, we follow prior work~\cite{easg2024,air_vqa2025} and avoid repeated cropping. Instead, we perform a single forward pass per frame and extract object feature representation maps directly from the model output.

\subsection{Graph representation}
\label{sec:graph_representations}

Each graph is converted to a tensor representation containing: the clip feature, a 1D verb index tensor, a 1D auxiliary verb index tensor, a 1D multi-hot object index vector, 2D object - attribute multi-hot vectors, 2D object - relation multi-hot vectors, object features, and a set of $(\text{verb}, \text{object}, \text{relation})$ triplets.

Using this tensor, we build a trainable action scene graph embedder that constructs a fixed size graph feature representation. Verbs, objects, and relations are embedded into fixed dimensional vectors, following the standard dictionary based embedding design~\cite{deshwal2023dictionaryembeddings}. Objects and their features, as well as auxiliary verbs, are pooled using Multi-Query Pooling~\cite{shazeer2019multiquery} to account for the fact that certain objects and auxiliary verbs are more informative when describing an action. The clip feature is optionally projected into a lower dimensional space, and triplets are projected into a embedding of fixed size using an MLP. The final graph representation is obtained by concatenating the resulting embeddings along the feature dimension to form a 1D graph descriptor.

Each input batch consists of frames obtained at times $t_i \ldots t_{i+9}$, forming a 10 frame activity window. The batch consists of per frame action annotations and object grounding, which are used to construct a graph at each timestamp, and a corresponding activity label for the whole 10 frame window. A full graph batch representation is shown in Appendix in Figure~\ref{}. The embedder is part of the graph model described in Section~\ref{sec:graph_model} and visualized in Figure~\ref{}.

\subsection{Graph-based model}
\label{sec:graph_model}

Our baselines consist of an MLP head trained on top of frozen vision features obtained from DINOv3~\cite{dinov3_2023} and TimeSformer~\cite{timesformer2021}. To ensure fair comparison with these vision representations, we also train only an MLP head on top of our graph representations, treating the ASG embedding as a structured alternative to the global visual feature, and do not employ a graph neural network.

Since each graph representation is a high-dimensional tensor with over 2500 dimensions, and since we have $N{=}10$ such graph representations across one activity window, this input is prone to the curse of dimensionality~\cite{peng2024curseofdimensionality}. We therefore project each graph embedding into a lower-dimensional output space and apply (self) attention pooling~\cite{bahdanau2015attention} across the temporal window to obtain a fixed shape activity representation. The resulting compact representation is then fed to an MLP classifier for activity recognition.

Given a batch of $B$ activity windows, each represented as a sequence of $N$ action scene graphs, the input is written as
$\{\mathcal{G}_{b,t}\}_{b=1,t=1}^{B,N}$.
Each graph $\mathcal{G}_{b,t}$ is mapped to a fixed-dimensional embedding by the \textsc{ActionGraphEmbedder}, producing
\begin{equation}
    \mathbf{H} = \mathrm{Embed}(\{\mathcal{G}_{b,t}\}) \in \mathbb{R}^{B \times N \times d},
\end{equation}
where $d$ denotes the embedding dimension, where $d_g \leq d$. Optionally, we apply a projection block (Linear $\rightarrow$ LayerNorm $\rightarrow$ GELU) to obtain
\begin{equation}
    \mathbf{H}_g = \mathrm{Proj}(\mathbf{H}) \in \mathbb{R}^{B \times N \times d_g}.
\end{equation}
To aggregate information across the temporal window, we apply attention pooling over the $N$ graph embeddings, obtaining an activity level representation
\begin{equation}
    \mathbf{z} = \mathrm{AttnPool}(\mathbf{H}_g) \in \mathbb{R}^{B \times d_p}.
\end{equation}
Finally, an MLP classifier predicts activity classes:
\begin{equation}
    \hat{\mathbf{y}} = \mathrm{MLP}(\mathbf{z}) \in \mathbb{R}^{B \times C},
\end{equation}
where $C$ denotes the number of activity classes and $\hat{\mathbf{y}}$ contains the per-class logits. A visualization of the module is shown in Figure~\ref{}.

